Towards Making a Trojan-horse Attack on Text-to-Image Retrieval

While deep learning based image retrieval is reported to be vulnerable to adversarial attacks, existing works are mainly on image-to-image retrieval with their attacks performed at the front end via query modification. By contrast, we present in this paper the first study about a threat that occurs at the back end of a text-to-image retrieval (T2IR) system. Our study is motivated by the fact that the image collection indexed by the system will be regularly updated due to the arrival of new images from various sources such as web crawlers and advertisers. With malicious images indexed, it is possible for an attacker to indirectly interfere with the retrieval process, letting users see certain images that are completely irrelevant w.r.t. their queries. We put this thought into practice by proposing a novel Trojan-horse attack (THA). In particular, we construct a set of Trojan-horse images by first embedding word-specific adversarial information into a QR code and then putting the code on benign advertising images. A proof-of-concept evaluation, conducted on two popular T2IR datasets (Flickr30k and MS-COCO), shows the effectiveness of the proposed THA in a white-box mode.

==> Image/Fig_adjust_lambda.tex <==
\begin{figure}[htbp!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=0.48\textwidth]{Image/qr_adjust_lam.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{\textbf{Attack performance with different $\lambda$ on {\TargetedObject} motorcycle and policeman.} LBIR  setup: CLIP + Flickr30ktest. Adversarial patches are learned with Flickr30ktrain as training data.} %最终文档中希望显示的图片标题
\label{Figure:adjust_lambda} %用于文内引用的标签
\end{figure}

==> Image/Fig_adjust_patch_ratio.tex <==
\begin{figure}[htbp!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=0.5\textwidth]{Image/adjust_ratio.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{\textbf{Attack performance (mean trojan-horse R10) with different patch ratio on Flickr30k.} 
% LBIR  setup: CLIP + Flickr30ktest. Adversarial patches are learned with Flickr30ktrain as training data.
} 
\label{Figure:adjust_patch_ratio} %用于文内引用的标签
\end{figure}

% \begin{figure}

%   \begin{subfigure}{0.49\linewidth} % 如果一行放2个图，用0.5，如果3个图，用0.33
%     \centering 
%     \includegraphics[scale=0.25]{Image/adjust_ratio1.pdf} 
%     \caption{jacket, sidewalk and dress}
%     \label{fig:adjust_patch_ratio1}
%   \end{subfigure}
%   \begin{subfigure}{0.49\linewidth}
%     \centering 
%     \includegraphics[scale=0.25]{Image/adjust_ratio2.pdf} 
%     \caption{glasses, female and policeman}
%     \label{fig:adjust_patch_ratio2}
%   \end{subfigure}
  
%  \caption{\textbf{Attack performance with different patch percentage on six concepts.}}
%   \label{Figure:adjust_patch_ratio}
% \end{figure}

==> Image/Fig_adjust_sigma.tex <==

\begin{figure}
    \subfloat[ CLIP+ ~  Flickr30ktest. \label{fig:adjust_sigma_clip_F}]{\includegraphics[width=0.5\columnwidth]{Image/adjust_sigma_clip_F.pdf}} 
    \subfloat[ {\clipF}+Flickr30ktest. \label{fig:adjust_sigma_clipft_F}]{\includegraphics[width=0.5\columnwidth]{Image/adjust_sigma_clipft_F.pdf}} 
    
    \subfloat[ CLIP+COCOtest. \label{fig:adjust_sigma_clip_C}]{\includegraphics[width=0.5\columnwidth]{Image/adjust_sigma_clip_C.pdf}} 
    \subfloat[ {\clipC}+COCOtest. \label{fig:adjust_sigma_clipft_C}]{\includegraphics[width=0.5\columnwidth]{Image/adjust_sigma_clipft_C.pdf}} 
    \caption{\textbf{Attack performance (mean trojan-horse R10) with different Gaussian's $\sigma$.}}
    \label{Figure:adjust_sigma}
\end{figure}

==> Image/Fig_adjust_sigma_origin.tex <==

\begin{figure}
    \subfloat[ CLIP+ ~  Flickr30ktest. \label{fig:adjust_sigma_clip_F_origin}]{\includegraphics[width=0.5\columnwidth]{Image/origin_adjust_sigma/clip_Flickr.pdf}} 
    \subfloat[ {\clipF}+Flickr30ktest. \label{fig:adjust_sigma_clipft_F_origin}]{\includegraphics[width=0.5\columnwidth]{Image/origin_adjust_sigma/clipft_Flickr.pdf}} 
    
    \subfloat[ CLIP+COCOtest. \label{fig:adjust_sigma_clip_C_origin}]{\includegraphics[width=0.5\columnwidth]{Image/origin_adjust_sigma/clip_COCO.pdf}} 
    \subfloat[ {\clipC}+COCOtest. \label{fig:adjust_sigma_clipft_C_origin}]{\includegraphics[width=0.5\columnwidth]{Image/origin_adjust_sigma/clipft_COCO.pdf}} 
    \caption{\textbf{Retrieval performance (mean Truly relevant R10) with different Gaussian's $\sigma$.}}
    \label{Figure:adjust_sigma_origin}
\end{figure}

==> Image/Fig_benign.tex <==
\begin{figure}[t!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=\columnwidth]{Image/benign_4x5.jpg} %插入图片，[]中设置图片大小，{}中是图片文件名
%\caption{\textbf{Overview of 20 benign images}. We randomly select 20 advertisement images from the Internet as the benign images.}
\caption{\textbf{Twenty benign images used in our experiments}, consisting of diverse advertisement images we randomly downloaded from the Internet. They act as carriers of our Trojan-horse attacks.}
%最终文档中希望显示的图片标题
\label{fig:benign} %用于文内引用的标签
\end{figure}


==> Image/Fig_pipeline_attack.tex <==
\begin{figure*}[htbp!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=1.0\textwidth]{Image/pipeline_attack.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{\textbf{A conceptual illustration of Trojan-horse image generation}. Given a specific word $w$ and a set of benign images $X_b$, we construct a set of Trojan-horse images $X_{h,w}$ by overlaying a word-specific adversarial patch $\delta$ on each image in $X_b$. The patch is derived by iteratively making an attack on an existing cross-modal matching network to enforce the Trojan-horse images to be more close to the given word in the cross-modal feature space.
%The attack pipeline: Input the sentences $S_w$ which contain the target {\TargetedObject} $w$ into the text encoder (BERT \cite{vaswani2017attention}) and the trojan-horse images $X_i$ which are generated by the i-th iteration adversarial patch $\delta_i $ into the image encoder (ViT \cite{ICLR_DosovitskiyB0WZ21}) of a language-based retrieval model. We get the 
%sentence embeddings $e(S_w)$ and the image embeddings $e(X_i)$. Then we design the loss function to minimize the distance between the contextualized deep embedding of {\TargetedObject} $e(w)$ and the trojan-horse embeddings $e(X_i)$ in the feature space. With the gradient of backpropagation, we get new adversarial patch $\delta_{i+1} $ for next iteration.
} %最终文档中希望显示的图片标题
\label{fig:training} %用于文内引用的标签
\end{figure*}

% 分别将含有target concept的sentences和第i次迭代后带有patch $\delta_i $ 的 trojan-horse images 输入retrieval model 生成的 句子的embeddings $e(T_c)$和图片的embeddings $e(X)$, 利用损失函数进行梯度回传(图中黑色箭头)，修改patch的像素值(i.e. 图中绿色虚线框标出部分)使 $e(T_c)$和 $e(X)$在feature space中更接近.

==> Image/Fig_pipeline_retrieval.tex <==
\begin{figure}[htbp!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=0.48\textwidth]{Image/pipeline_retrieval.jpg} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{\textbf{The pipeline of targeted Trojan-Horse Attacks on Language-based Image Retrieval}. } %最终文档中希望显示的图片标题
\label{Figure:pipeline_retrieval} %用于文内引用的标签
\end{figure}

% 分别将含有target concept的sentences和带有patch的adversarial images输入retrieval model 生成的 句子的embeddings $e(T_c)$和图片的embeddings $e(X)$, 利用损失函数进行梯度回传(图中黑色箭头)，修改patch的像素值(i.e. 图中绿色虚线框标出部分)使 $e(T_c)$和 $e(X)$在feature space中更接近.


%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{Image/pipeline_retrieval.jpg}
%   \caption{\textbf{Overview of targeted Trojan-Horse Attacks on Language-based Image Retrieval cross-modal retrieval systems}. }
%   \Description{Enjoying the baseball game from the third-base seats. Ichiro Suzuki preparing to bat.}
%   \label{Figure:pipeline_retrieval}
% \end{teaserfigure}


==> Image/Fig_result_visualization.tex <==
% \begin{figure*}[htbp!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
% \centering %图片居中
% \includegraphics[width=1.0\textwidth]{Image/result_visualization.png} %插入图片，[]中设置图片大小，{}中是图片文件名
% \caption{Two examples of attacking  Language-based Image Retrieval system. Note that images in red frames indicate that they are trojan-horse images.} %最终文档中希望显示的图片标题
% \label{Figure:resulti_visualization} %用于文内引用的标签
% \end{figure*}

%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
% \begin{teaserfigure}
%   \includegraphics[width=1.0\textwidth]{Image/result_visualization.png}
%   \caption{Two examples of attacking  Language-based Image Retrieval system. Note that images in red frames indicate that they are trojan-horse images.}
%   \label{Figure:resulti_visualization}
% \end{teaserfigure}

==> Image/Fig_tsne.tex <==
\begin{figure}

  \begin{subfigure}{0.49\linewidth} % 如果一行放2个图，用0.5，如果3个图，用0.33
    \centering 
    \includegraphics[scale=0.25]{Image/policeman_Tsne_result.jpg} 
    \caption{policeman}
    \label{fig:tsne_policeman}
  \end{subfigure}
  \begin{subfigure}{0.49\linewidth}
    \centering 
    \includegraphics[scale=0.25]{Image/swimming_Tsne_result.jpg} 
    \caption{swimming}
    \label{fig:tsne_swimming}
  \end{subfigure}
  
  \begin{subfigure}{0.49\linewidth}
    \centering 
    \includegraphics[scale=0.25]{Image/front_Tsne_result.jpg} 
    \caption{front}
    \label{fig:tsne_front}
  \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
    \centering 
    \includegraphics[scale=0.25]{Image/run_Tsne_result.jpg} 
    \caption{run}
    \label{fig:tsne_runs}
  \end{subfigure}
  
 \caption{\textbf{Visualization of {\clipF} model embbedings of four {\TargetedObject}s in Flickr30Ktest. } Grey dots, purple dots, and yellow dots mean all images in test dataset, texts including targeted {\TargetedObject}  in test dataset and trojan-horse images. }
  \label{Figure:tsne_four_concepts}
\end{figure}

==> Image/Fig_visualization_adjust_ratio.tex <==
\begin{figure}[t!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=0.5\textwidth]{Image/visualization_adjust_ratio.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{\textbf{Visualization of different patch percentage for {\TargetedObject} jacket.} LBIR  setup: {\clipF} + Flickr30ktest. Adversarial patches are learned with Flickr30ktrain as training data.} %最终文档中希望显示的图片标题
\label{Figure:visualization_adjust_ratio} %用于文内引用的标签
\end{figure}



==> Image/Fig_visualization_adjust_sigma.tex <==
\begin{figure*}[t!] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中
\includegraphics[width=1.0\textwidth]{Image/visualization_adjust_sigma.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{\textbf{Visualization of different Gaussian’s $\sigma$.} LBIR  setup: {CLIP} + Flickr30ktest. Adversarial patches are learned with Flickr30ktrain as training data.} %最终文档中希望显示的图片标题
\label{Figure:visualization_adjust_sigma} %用于文内引用的标签
\end{figure*}



==> Table/ICASSP_deleted_table.tex <==
\subsection{fully white-box setup}
\begin{table}[thb!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\centering
\caption{\textbf{Evaluating THA in a fully white-box setup}. Metric: Recall at 10 (R10). Lower recall scores of relevant images and higher recall scores of TH images are better.}
\scalebox{1.0}{
\begin{tabular}{@{}lcrr@{}}
\toprule
\textbf{T2IR model} & \textbf{THA} & \multicolumn{1}{l}{\textbf{Rel. images  ($\downarrow$)}} & \multicolumn{1}{l}{\textbf{Benign / TH  ($\uparrow$)}} \\ \midrule
\multicolumn{4}{@{}l}{\textit{Dataset: Flickr30k}} \\ 
CLIP & - & 94.9 & 0.0 \\
CLIP & + & 52.1 & 97.2 \\
{\clipF} & -  & 98.6 & 0.8 \\
{\clipF} & +  & 95.3 & 77.1 \\ \midrule
\multicolumn{4}{@{}l}{\textit{Dataset: COCO}} \\
CLIP & - & 80.5 & 0.0 \\
CLIP & +  & 51.2 & 82.3 \\
{\clipC} & - & 90.1 & 1.8 \\
{\clipC} & + & 83.9 & 44.9 \\
\bottomrule
\end{tabular}
}\label{tab:result_white_box}

\end{table}


\subsection{cross-dataset setup}
\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\centering
\caption{\textbf{Evaluating THA in a cross-dataset setup}.
%, where COCO (Flickr30k) is used for TH image generation and T2IR is performed on Flickr30k (COCO).
}
\begin{center}
\scalebox{1}{
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{T2IR model} & \multicolumn{1}{l}{\textbf{Rel. images  ($\downarrow$)}} & \multicolumn{1}{r}{\textbf{TH images ($\uparrow$)}} \\ \midrule
\multicolumn{3}{@{}l}{\textit{T2IR on Flickr30k, with TH generation using COCO}:} \\ [2pt]
CLIP  & 70.5 & 83.1 \\
{\clipF} & 97.7 & 58.6 \\
%{\clipC} & 94.8 & 69.2 \\ 
\midrule
\multicolumn{3}{@{}l}{\textit{T2IR on COCO, with TH generation using Flickr30k:}} \\ [2pt] 
CLIP  & 53.5 & 77.8 \\
%{\clipF}  & 82.8 & 34.4 \\
{\clipC} & 84.0 & 44.5 \\
\bottomrule
\end{tabular}
}
\end{center}

\label{tab:result_cross_dataset}

\end{table}



==> Table/all_result.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\newcommand{\ScaleNum}{0.65}

\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{Targeted attack performance of 24 {\TargetedObject}s for CLIP~\cite{2021clip_icml} on Flickr30k}. }
\begin{center}
\scalebox{\ScaleNum}{

\begin{tabular}{|l|ll|ll|ll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Keyword}} & \multicolumn{2}{c|}{Truly relevant (mAP)} & \multicolumn{2}{c|}{Truly relevant (R10)} & \multicolumn{2}{c|}{Trojan} & \multicolumn{2}{c|}{Trojan (R10)} \\ \cline{2-9} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after \\ \hline
waiter & \multicolumn{1}{l|}{1.000} & 0.238 & \multicolumn{1}{l|}{100.0} & 20.0 & \multicolumn{1}{l|}{0.012} & 0.961 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
climbing & \multicolumn{1}{l|}{0.630} & 0.126 & \multicolumn{1}{l|}{95.5} & 11.4 & \multicolumn{1}{l|}{0.010} & 0.945 & \multicolumn{1}{l|}{0.0} & 97.7 \\ \hline
motorcycle & \multicolumn{1}{l|}{0.745} & 0.143 & \multicolumn{1}{l|}{90.5} & 28.6 & \multicolumn{1}{l|}{0.010} & 0.932 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
little & \multicolumn{1}{l|}{0.766} & 0.212 & \multicolumn{1}{l|}{91.9} & 29.0 & \multicolumn{1}{l|}{0.010} & 0.927 & \multicolumn{1}{l|}{0.0} & 98.9 \\ \hline
run & \multicolumn{1}{l|}{0.622} & 0.152 & \multicolumn{1}{l|}{92.3} & 30.8 & \multicolumn{1}{l|}{0.010} & 0.913 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
dress & \multicolumn{1}{l|}{0.721} & 0.295 & \multicolumn{1}{l|}{92.4} & 42.4 & \multicolumn{1}{l|}{0.010} & 0.888 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
cow & \multicolumn{1}{l|}{0.956} & 0.635 & \multicolumn{1}{l|}{100.0} & 73.3 & \multicolumn{1}{l|}{0.010} & 0.885 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
feeding & \multicolumn{1}{l|}{0.900} & 0.621 & \multicolumn{1}{l|}{100.0} & 60.0 & \multicolumn{1}{l|}{0.010} & 0.871 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
floating & \multicolumn{1}{l|}{0.820} & 0.382 & \multicolumn{1}{l|}{90.0} & 40.0 & \multicolumn{1}{l|}{0.012} & 0.870 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
policeman & \multicolumn{1}{l|}{0.806} & 0.496 & \multicolumn{1}{l|}{100.0} & 58.3 & \multicolumn{1}{l|}{0.010} & 0.864 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
dancing & \multicolumn{1}{l|}{0.534} & 0.257 & \multicolumn{1}{l|}{80.0} & 33.3 & \multicolumn{1}{l|}{0.011} & 0.864 & \multicolumn{1}{l|}{0.0} & 96.7 \\ \hline
reading & \multicolumn{1}{l|}{0.868} & 0.368 & \multicolumn{1}{l|}{94.7} & 52.6 & \multicolumn{1}{l|}{0.011} & 0.832 & \multicolumn{1}{l|}{0.0} & 94.7 \\ \hline
smiling & \multicolumn{1}{l|}{0.761} & 0.427 & \multicolumn{1}{l|}{94.6} & 48.2 & \multicolumn{1}{l|}{0.011} & 0.829 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
floor & \multicolumn{1}{l|}{0.901} & 0.519 & \multicolumn{1}{l|}{97.7} & 70.5 & \multicolumn{1}{l|}{0.011} & 0.814 & \multicolumn{1}{l|}{0.0} & 95.5 \\ \hline
swimming & \multicolumn{1}{l|}{0.726} & 0.289 & \multicolumn{1}{l|}{97.8} & 43.5 & \multicolumn{1}{l|}{0.011} & 0.812 & \multicolumn{1}{l|}{0.0} & 97.8 \\ \hline
pink & \multicolumn{1}{l|}{0.765} & 0.430 & \multicolumn{1}{l|}{94.3} & 52.9 & \multicolumn{1}{l|}{0.011} & 0.796 & \multicolumn{1}{l|}{0.0} & 94.3 \\ \hline
blue & \multicolumn{1}{l|}{0.753} & 0.465 & \multicolumn{1}{l|}{95.4} & 61.4 & \multicolumn{1}{l|}{0.010} & 0.755 & \multicolumn{1}{l|}{0.0} & 97.3 \\ \hline
navy & \multicolumn{1}{l|}{0.792} & 0.538 & \multicolumn{1}{l|}{100.0} & 66.7 & \multicolumn{1}{l|}{0.011} & 0.742 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
yellow & \multicolumn{1}{l|}{0.752} & 0.519 & \multicolumn{1}{l|}{93.2} & 68.9 & \multicolumn{1}{l|}{0.011} & 0.699 & \multicolumn{1}{l|}{0.0} & 96.3 \\ \hline
female & \multicolumn{1}{l|}{0.728} & 0.467 & \multicolumn{1}{l|}{100.0} & 73.9 & \multicolumn{1}{l|}{0.011} & 0.676 & \multicolumn{1}{l|}{0.0} & 89.1 \\ \hline
jacket & \multicolumn{1}{l|}{0.728} & 0.538 & \multicolumn{1}{l|}{91.4} & 69.9 & \multicolumn{1}{l|}{0.011} & 0.666 & \multicolumn{1}{l|}{0.0} & 94.6 \\ \hline
green & \multicolumn{1}{l|}{0.789} & 0.590 & \multicolumn{1}{l|}{94.9} & 76.0 & \multicolumn{1}{l|}{0.010} & 0.625 & \multicolumn{1}{l|}{0.0} & 92.0 \\ \hline
maroon & \multicolumn{1}{l|}{0.729} & 0.627 & \multicolumn{1}{l|}{100.0} & 60.0 & \multicolumn{1}{l|}{0.011} & 0.602 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
front & \multicolumn{1}{l|}{0.713} & 0.566 & \multicolumn{1}{l|}{92.0} & 78.0 & \multicolumn{1}{l|}{0.011} & 0.561 & \multicolumn{1}{l|}{0.0} & 88.6 \\ \hline
\textbf{MEAN} & \multicolumn{1}{l|}{\textbf{0.771}} & \textbf{0.413} & \multicolumn{1}{l|}{\textbf{94.9}} & \textbf{52.1} & \multicolumn{1}{l|}{\textbf{0.011}} & \textbf{0.805} & \multicolumn{1}{l|}{\textbf{0.0}} & \textbf{97.2} \\ \hline
\end{tabular}

}
\end{center}

\label{tab:result_F_C}

\end{table}



\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{Targeted attack performance of 24 {\TargetedObject}s for {\clipF}}. }
\begin{center}
\scalebox{\ScaleNum}{

\begin{tabular}{|l|ll|ll|ll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Keyword}} & \multicolumn{2}{c|}{Truly relevant (mAP)} & \multicolumn{2}{c|}{Truly relevant (R10)} & \multicolumn{2}{c|}{Trojan} & \multicolumn{2}{c|}{Trojan (R10)} \\ \cline{2-9} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after \\ \hline
cow & \multicolumn{1}{l|}{1.000} & 0.877 & \multicolumn{1}{l|}{100.0} & 86.7 & \multicolumn{1}{l|}{0.017} & 0.862 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
motorcycle & \multicolumn{1}{l|}{0.976} & 0.825 & \multicolumn{1}{l|}{100.0} & 95.2 & \multicolumn{1}{l|}{0.020} & 0.818 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
policeman & \multicolumn{1}{l|}{0.958} & 0.836 & \multicolumn{1}{l|}{100.0} & 100.0 & \multicolumn{1}{l|}{0.017} & 0.793 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
reading & \multicolumn{1}{l|}{0.894} & 0.786 & \multicolumn{1}{l|}{94.7} & 86.8 & \multicolumn{1}{l|}{0.024} & 0.766 & \multicolumn{1}{l|}{0.0} & 97.4 \\ \hline
waiter & \multicolumn{1}{l|}{1.000} & 1.000 & \multicolumn{1}{l|}{100.0} & 100.0 & \multicolumn{1}{l|}{0.027} & 0.756 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
climbing & \multicolumn{1}{l|}{0.822} & 0.636 & \multicolumn{1}{l|}{95.5} & 84.1 & \multicolumn{1}{l|}{0.016} & 0.682 & \multicolumn{1}{l|}{0.0} & 84.1 \\ \hline
floor & \multicolumn{1}{l|}{0.966} & 0.949 & \multicolumn{1}{l|}{100.0} & 100.0 & \multicolumn{1}{l|}{0.019} & 0.669 & \multicolumn{1}{l|}{2.3} & 86.4 \\ \hline
dress & \multicolumn{1}{l|}{0.852} & 0.781 & \multicolumn{1}{l|}{100.0} & 95.5 & \multicolumn{1}{l|}{0.020} & 0.626 & \multicolumn{1}{l|}{1.5} & 86.4 \\ \hline
feeding & \multicolumn{1}{l|}{1.000} & 1.000 & \multicolumn{1}{l|}{100.0} & 100.0 & \multicolumn{1}{l|}{0.016} & 0.612 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
swimming & \multicolumn{1}{l|}{0.828} & 0.771 & \multicolumn{1}{l|}{100.0} & 100.0 & \multicolumn{1}{l|}{0.021} & 0.611 & \multicolumn{1}{l|}{0.0} & 91.3 \\ \hline
floating & \multicolumn{1}{l|}{0.920} & 0.904 & \multicolumn{1}{l|}{100.0} & 90.0 & \multicolumn{1}{l|}{0.026} & 0.585 & \multicolumn{1}{l|}{0.0} & 70.0 \\ \hline
dancing & \multicolumn{1}{l|}{0.739} & 0.684 & \multicolumn{1}{l|}{90.0} & 83.3 & \multicolumn{1}{l|}{0.018} & 0.544 & \multicolumn{1}{l|}{0.0} & 83.3 \\ \hline
pink & \multicolumn{1}{l|}{0.918} & 0.893 & \multicolumn{1}{l|}{97.7} & 96.6 & \multicolumn{1}{l|}{0.019} & 0.538 & \multicolumn{1}{l|}{0.0} & 86.2 \\ \hline
yellow & \multicolumn{1}{l|}{0.891} & 0.873 & \multicolumn{1}{l|}{97.5} & 93.8 & \multicolumn{1}{l|}{0.025} & 0.534 & \multicolumn{1}{l|}{3.1} & 77.6 \\ \hline
navy & \multicolumn{1}{l|}{0.917} & 0.917 & \multicolumn{1}{l|}{100.0} & 100.0 & \multicolumn{1}{l|}{0.018} & 0.531 & \multicolumn{1}{l|}{0.0} & 66.7 \\ \hline
smiling & \multicolumn{1}{l|}{0.883} & 0.862 & \multicolumn{1}{l|}{100.0} & 98.2 & \multicolumn{1}{l|}{0.023} & 0.482 & \multicolumn{1}{l|}{3.6} & 83.9 \\ \hline
green & \multicolumn{1}{l|}{0.908} & 0.894 & \multicolumn{1}{l|}{98.9} & 97.1 & \multicolumn{1}{l|}{0.017} & 0.453 & \multicolumn{1}{l|}{0.6} & 73.1 \\ \hline
run & \multicolumn{1}{l|}{0.808} & 0.773 & \multicolumn{1}{l|}{100.0} & 92.3 & \multicolumn{1}{l|}{0.019} & 0.386 & \multicolumn{1}{l|}{0.0} & 69.2 \\ \hline
jacket & \multicolumn{1}{l|}{0.880} & 0.873 & \multicolumn{1}{l|}{96.8} & 95.7 & \multicolumn{1}{l|}{0.022} & 0.364 & \multicolumn{1}{l|}{0.0} & 57.0 \\ \hline
little & \multicolumn{1}{l|}{0.896} & 0.882 & \multicolumn{1}{l|}{98.9} & 98.4 & \multicolumn{1}{l|}{0.017} & 0.362 & \multicolumn{1}{l|}{1.1} & 65.6 \\ \hline
maroon & \multicolumn{1}{l|}{0.867} & 0.867 & \multicolumn{1}{l|}{100.0} & 100.0 & \multicolumn{1}{l|}{0.022} & 0.342 & \multicolumn{1}{l|}{0.0} & 40.0 \\ \hline
female & \multicolumn{1}{l|}{0.942} & 0.942 & \multicolumn{1}{l|}{100.0} & 100.0 & \multicolumn{1}{l|}{0.023} & 0.329 & \multicolumn{1}{l|}{2.2} & 60.9 \\ \hline
blue & \multicolumn{1}{l|}{0.886} & 0.885 & \multicolumn{1}{l|}{98.2} & 97.9 & \multicolumn{1}{l|}{0.018} & 0.287 & \multicolumn{1}{l|}{1.2} & 41.6 \\ \hline
front & \multicolumn{1}{l|}{0.859} & 0.857 & \multicolumn{1}{l|}{97.3} & 96.6 & \multicolumn{1}{l|}{0.023} & 0.200 & \multicolumn{1}{l|}{4.2} & 29.9 \\ \hline
\textbf{MEAN} & \multicolumn{1}{l|}{\textbf{0.900}} & \textbf{0.857} & \multicolumn{1}{l|}{\textbf{98.6}} & \textbf{95.3} & \multicolumn{1}{l|}{\textbf{0.020}} & \textbf{0.547} & \multicolumn{1}{l|}{\textbf{0.8}} & \textbf{77.1} \\ \hline
\end{tabular}

}
\end{center}

\label{tab:result_F_C-FT}

\end{table}



\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{Targeted attack performance of 24 {\TargetedObject}s for CLIP~\cite{2021clip_icml} on MSCOCO}. }
\begin{center}
\scalebox{\ScaleNum}{

\begin{tabular}{|l|ll|ll|ll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Keyword}} & \multicolumn{2}{c|}{Truly relevant (mAP)} & \multicolumn{2}{c|}{Truly relevant (R10)} & \multicolumn{2}{c|}{Trojan} & \multicolumn{2}{c|}{Trojan (R10)} \\ \cline{2-9} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after \\ \hline
waiter & \multicolumn{1}{l|}{0.333} & 0.045 & \multicolumn{1}{l|}{100.0} & 0.0 & \multicolumn{1}{l|}{0.002} & 0.992 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
policeman & \multicolumn{1}{l|}{0.712} & 0.234 & \multicolumn{1}{l|}{80.0} & 20.0 & \multicolumn{1}{l|}{0.002} & 0.965 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
dancing & \multicolumn{1}{l|}{0.625} & 0.524 & \multicolumn{1}{l|}{100.0} & 50.0 & \multicolumn{1}{l|}{0.002} & 0.854 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
floating & \multicolumn{1}{l|}{0.354} & 0.107 & \multicolumn{1}{l|}{68.4} & 18.4 & \multicolumn{1}{l|}{0.003} & 0.842 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
maroon & \multicolumn{1}{l|}{0.540} & 0.165 & \multicolumn{1}{l|}{100.0} & 60.0 & \multicolumn{1}{l|}{0.002} & 0.792 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
smiling & \multicolumn{1}{l|}{0.503} & 0.228 & \multicolumn{1}{l|}{77.6} & 35.8 & \multicolumn{1}{l|}{0.003} & 0.791 & \multicolumn{1}{l|}{0.0} & 97.8 \\ \hline
motorcycle & \multicolumn{1}{l|}{0.387} & 0.207 & \multicolumn{1}{l|}{62.7} & 31.5 & \multicolumn{1}{l|}{0.002} & 0.776 & \multicolumn{1}{l|}{0.0} & 98.1 \\ \hline
little & \multicolumn{1}{l|}{0.587} & 0.245 & \multicolumn{1}{l|}{82.4} & 34.5 & \multicolumn{1}{l|}{0.002} & 0.775 & \multicolumn{1}{l|}{0.0} & 87.9 \\ \hline
pink & \multicolumn{1}{l|}{0.689} & 0.526 & \multicolumn{1}{l|}{89.7} & 68.4 & \multicolumn{1}{l|}{0.002} & 0.641 & \multicolumn{1}{l|}{0.0} & 94.1 \\ \hline
cow & \multicolumn{1}{l|}{0.513} & 0.370 & \multicolumn{1}{l|}{76.4} & 52.8 & \multicolumn{1}{l|}{0.002} & 0.626 & \multicolumn{1}{l|}{0.0} & 95.3 \\ \hline
dress & \multicolumn{1}{l|}{0.572} & 0.289 & \multicolumn{1}{l|}{88.7} & 52.8 & \multicolumn{1}{l|}{0.002} & 0.619 & \multicolumn{1}{l|}{0.0} & 84.9 \\ \hline
reading & \multicolumn{1}{l|}{0.745} & 0.490 & \multicolumn{1}{l|}{93.6} & 70.2 & \multicolumn{1}{l|}{0.002} & 0.595 & \multicolumn{1}{l|}{0.0} & 78.7 \\ \hline
climbing & \multicolumn{1}{l|}{0.483} & 0.331 & \multicolumn{1}{l|}{94.1} & 58.8 & \multicolumn{1}{l|}{0.002} & 0.564 & \multicolumn{1}{l|}{0.0} & 88.2 \\ \hline
jacket & \multicolumn{1}{l|}{0.456} & 0.291 & \multicolumn{1}{l|}{75.0} & 53.1 & \multicolumn{1}{l|}{0.002} & 0.530 & \multicolumn{1}{l|}{0.0} & 87.5 \\ \hline
navy & \multicolumn{1}{l|}{0.518} & 0.295 & \multicolumn{1}{l|}{83.3} & 66.7 & \multicolumn{1}{l|}{0.002} & 0.529 & \multicolumn{1}{l|}{0.0} & 83.3 \\ \hline
swimming & \multicolumn{1}{l|}{0.728} & 0.573 & \multicolumn{1}{l|}{93.5} & 78.3 & \multicolumn{1}{l|}{0.002} & 0.508 & \multicolumn{1}{l|}{0.0} & 80.4 \\ \hline
blue & \multicolumn{1}{l|}{0.502} & 0.393 & \multicolumn{1}{l|}{75.0} & 60.4 & \multicolumn{1}{l|}{0.002} & 0.450 & \multicolumn{1}{l|}{0.0} & 65.5 \\ \hline
yellow & \multicolumn{1}{l|}{0.530} & 0.419 & \multicolumn{1}{l|}{78.6} & 63.6 & \multicolumn{1}{l|}{0.003} & 0.448 & \multicolumn{1}{l|}{0.0} & 70.9 \\ \hline
floor & \multicolumn{1}{l|}{0.608} & 0.443 & \multicolumn{1}{l|}{85.8} & 67.6 & \multicolumn{1}{l|}{0.003} & 0.442 & \multicolumn{1}{l|}{0.0} & 64.2 \\ \hline
feeding & \multicolumn{1}{l|}{0.523} & 0.446 & \multicolumn{1}{l|}{76.4} & 69.1 & \multicolumn{1}{l|}{0.002} & 0.415 & \multicolumn{1}{l|}{0.0} & 56.4 \\ \hline
female & \multicolumn{1}{l|}{0.329} & 0.245 & \multicolumn{1}{l|}{64.4} & 46.7 & \multicolumn{1}{l|}{0.003} & 0.358 & \multicolumn{1}{l|}{0.0} & 77.8 \\ \hline
run & \multicolumn{1}{l|}{0.209} & 0.154 & \multicolumn{1}{l|}{45.5} & 39.4 & \multicolumn{1}{l|}{0.002} & 0.333 & \multicolumn{1}{l|}{0.0} & 72.7 \\ \hline
green & \multicolumn{1}{l|}{0.478} & 0.444 & \multicolumn{1}{l|}{72.1} & 66.5 & \multicolumn{1}{l|}{0.002} & 0.243 & \multicolumn{1}{l|}{0.0} & 45.4 \\ \hline
front & \multicolumn{1}{l|}{0.460} & 0.424 & \multicolumn{1}{l|}{68.8} & 64.8 & \multicolumn{1}{l|}{0.002} & 0.231 & \multicolumn{1}{l|}{0.0} & 47.0 \\ \hline
\textbf{MEAN} & \multicolumn{1}{l|}{\textbf{0.516}} & \textbf{0.329} & \multicolumn{1}{l|}{\textbf{80.5}} & \textbf{51.2} & \multicolumn{1}{l|}{\textbf{0.002}} & \textbf{0.597} & \multicolumn{1}{l|}{\textbf{0.0}} & \textbf{82.3} \\ \hline
\end{tabular}

}
\end{center}

\label{tab:result_M_C}

\end{table}



\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{Targeted attack performance of 24 {\TargetedObject}s for {\clipC}}. }
\begin{center}
\scalebox{\ScaleNum}{

\begin{tabular}{|l|ll|ll|ll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Keyword}} & \multicolumn{2}{c|}{Truly relevant (mAP)} & \multicolumn{2}{c|}{Truly relevant (R10)} & \multicolumn{2}{c|}{Trojan} & \multicolumn{2}{c|}{Trojan (R10)} \\ \cline{2-9} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after & \multicolumn{1}{l|}{before} & after \\ \hline
waiter & \multicolumn{1}{l|}{1.000} & 0.250 & \multicolumn{1}{l|}{100.0} & 100.0 & \multicolumn{1}{l|}{0.003} & 0.922 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
policeman & \multicolumn{1}{l|}{0.381} & 0.244 & \multicolumn{1}{l|}{80.0} & 40.0 & \multicolumn{1}{l|}{0.004} & 0.806 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
dancing & \multicolumn{1}{l|}{0.600} & 0.520 & \multicolumn{1}{l|}{100.0} & 50.0 & \multicolumn{1}{l|}{0.008} & 0.762 & \multicolumn{1}{l|}{0.0} & 100.0 \\ \hline
navy & \multicolumn{1}{l|}{0.649} & 0.649 & \multicolumn{1}{l|}{83.3} & 83.3 & \multicolumn{1}{l|}{0.004} & 0.597 & \multicolumn{1}{l|}{0.0} & 83.3 \\ \hline
maroon & \multicolumn{1}{l|}{0.643} & 0.618 & \multicolumn{1}{l|}{80.0} & 60.0 & \multicolumn{1}{l|}{0.007} & 0.507 & \multicolumn{1}{l|}{20.0} & 80.0 \\ \hline
pink & \multicolumn{1}{l|}{0.825} & 0.773 & \multicolumn{1}{l|}{94.1} & 86.0 & \multicolumn{1}{l|}{0.007} & 0.470 & \multicolumn{1}{l|}{0.0} & 68.4 \\ \hline
reading & \multicolumn{1}{l|}{0.887} & 0.851 & \multicolumn{1}{l|}{97.9} & 91.5 & \multicolumn{1}{l|}{0.010} & 0.442 & \multicolumn{1}{l|}{6.4} & 57.4 \\ \hline
motorcycle & \multicolumn{1}{l|}{0.613} & 0.587 & \multicolumn{1}{l|}{86.8} & 77.8 & \multicolumn{1}{l|}{0.005} & 0.423 & \multicolumn{1}{l|}{0.0} & 54.0 \\ \hline
dress & \multicolumn{1}{l|}{0.764} & 0.734 & \multicolumn{1}{l|}{98.1} & 94.3 & \multicolumn{1}{l|}{0.007} & 0.371 & \multicolumn{1}{l|}{1.9} & 56.6 \\ \hline
cow & \multicolumn{1}{l|}{0.625} & 0.609 & \multicolumn{1}{l|}{90.6} & 86.6 & \multicolumn{1}{l|}{0.004} & 0.368 & \multicolumn{1}{l|}{0.0} & 45.7 \\ \hline
swimming & \multicolumn{1}{l|}{0.735} & 0.735 & \multicolumn{1}{l|}{97.8} & 97.8 & \multicolumn{1}{l|}{0.005} & 0.337 & \multicolumn{1}{l|}{0.0} & 32.6 \\ \hline
smiling & \multicolumn{1}{l|}{0.786} & 0.776 & \multicolumn{1}{l|}{95.5} & 94.0 & \multicolumn{1}{l|}{0.008} & 0.308 & \multicolumn{1}{l|}{0.7} & 44.0 \\ \hline
feeding & \multicolumn{1}{l|}{0.664} & 0.663 & \multicolumn{1}{l|}{89.1} & 89.1 & \multicolumn{1}{l|}{0.004} & 0.265 & \multicolumn{1}{l|}{1.8} & 38.2 \\ \hline
yellow & \multicolumn{1}{l|}{0.739} & 0.737 & \multicolumn{1}{l|}{92.4} & 92.0 & \multicolumn{1}{l|}{0.007} & 0.264 & \multicolumn{1}{l|}{1.2} & 30.6 \\ \hline
little & \multicolumn{1}{l|}{0.725} & 0.717 & \multicolumn{1}{l|}{93.1} & 92.4 & \multicolumn{1}{l|}{0.005} & 0.233 & \multicolumn{1}{l|}{0.3} & 37.9 \\ \hline
floating & \multicolumn{1}{l|}{0.492} & 0.488 & \multicolumn{1}{l|}{76.3} & 73.7 & \multicolumn{1}{l|}{0.006} & 0.224 & \multicolumn{1}{l|}{2.6} & 26.3 \\ \hline
floor & \multicolumn{1}{l|}{0.706} & 0.691 & \multicolumn{1}{l|}{92.0} & 90.9 & \multicolumn{1}{l|}{0.005} & 0.212 & \multicolumn{1}{l|}{1.1} & 25.6 \\ \hline
climbing & \multicolumn{1}{l|}{0.706} & 0.703 & \multicolumn{1}{l|}{94.1} & 94.1 & \multicolumn{1}{l|}{0.004} & 0.206 & \multicolumn{1}{l|}{0.0} & 23.5 \\ \hline
blue & \multicolumn{1}{l|}{0.706} & 0.702 & \multicolumn{1}{l|}{91.5} & 89.9 & \multicolumn{1}{l|}{0.006} & 0.191 & \multicolumn{1}{l|}{0.2} & 21.3 \\ \hline
jacket & \multicolumn{1}{l|}{0.697} & 0.696 & \multicolumn{1}{l|}{89.1} & 89.1 & \multicolumn{1}{l|}{0.007} & 0.185 & \multicolumn{1}{l|}{0.0} & 25.0 \\ \hline
green & \multicolumn{1}{l|}{0.652} & 0.645 & \multicolumn{1}{l|}{89.3} & 88.9 & \multicolumn{1}{l|}{0.004} & 0.144 & \multicolumn{1}{l|}{0.4} & 14.6 \\ \hline
female & \multicolumn{1}{l|}{0.537} & 0.537 & \multicolumn{1}{l|}{84.4} & 84.4 & \multicolumn{1}{l|}{0.008} & 0.100 & \multicolumn{1}{l|}{4.4} & 4.4 \\ \hline
run & \multicolumn{1}{l|}{0.446} & 0.446 & \multicolumn{1}{l|}{78.8} & 78.8 & \multicolumn{1}{l|}{0.004} & 0.060 & \multicolumn{1}{l|}{0.0} & 3.0 \\ \hline
front & \multicolumn{1}{l|}{0.644} & 0.642 & \multicolumn{1}{l|}{87.8} & 87.8 & \multicolumn{1}{l|}{0.007} & 0.044 & \multicolumn{1}{l|}{1.0} & 4.5 \\ \hline
\textbf{MEAN} & \multicolumn{1}{l|}{\textbf{0.676}} & \textbf{0.626} & \multicolumn{1}{l|}{\textbf{90.1}} & \textbf{83.9} & \multicolumn{1}{l|}{\textbf{0.006}} & \textbf{0.352} & \multicolumn{1}{l|}{\textbf{1.8}} & \textbf{44.9} \\ \hline
\end{tabular}

}
\end{center}

\label{tab:result_M_C-FT}

\end{table}


==> Table/concept_description.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{The class and mean cosine similarity (MCS) of 24 {\TargetedObject}s}.}
\begin{center}
\scalebox{1.0}{

\begin{tabular}{|l|c|ll|ll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Keyword}} & \multirow{2}{*}{Class} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Flickr30k \\ (1K test set)\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}MSCOCO \\ (5K test set)\end{tabular}} \\ \cline{3-6} 
\multicolumn{1}{|c|}{} &  & \multicolumn{1}{l|}{CLIP} & {\clipF} & \multicolumn{1}{l|}{CLIP} & {\clipC} \\ \hline
jacket & \multirow{8}{*}{noun} & \multicolumn{1}{l|}{0.693} & 0.403 & \multicolumn{1}{l|}{0.741} & 0.439 \\ \cline{1-1} \cline{3-6} 
dress &  & \multicolumn{1}{l|}{0.731} & 0.516 & \multicolumn{1}{l|}{0.728} & 0.507 \\ \cline{1-1} \cline{3-6} 
floor &  & \multicolumn{1}{l|}{0.776} & 0.565 & \multicolumn{1}{l|}{0.754} & 0.47 \\ \cline{1-1} \cline{3-6} 
female &  & \multicolumn{1}{l|}{0.735} & 0.411 & \multicolumn{1}{l|}{0.789} & 0.533 \\ \cline{1-1} \cline{3-6} 
motorcycle &  & \multicolumn{1}{l|}{0.831} & 0.665 & \multicolumn{1}{l|}{0.834} & 0.58 \\ \cline{1-1} \cline{3-6} 
policeman &  & \multicolumn{1}{l|}{0.849} & 0.716 & \multicolumn{1}{l|}{0.918} & 0.853 \\ \cline{1-1} \cline{3-6} 
cow &  & \multicolumn{1}{l|}{0.798} & 0.679 & \multicolumn{1}{l|}{0.827} & 0.633 \\ \cline{1-1} \cline{3-6} 
waiter &  & \multicolumn{1}{l|}{0.927} & 0.922 & \multicolumn{1}{l|}{1} & 1 \\ \hline
smiling & \multirow{8}{*}{verb} & \multicolumn{1}{l|}{0.711} & 0.474 & \multicolumn{1}{l|}{0.774} & 0.558 \\ \cline{1-1} \cline{3-6} 
climbing &  & \multicolumn{1}{l|}{0.812} & 0.588 & \multicolumn{1}{l|}{0.745} & 0.499 \\ \cline{1-1} \cline{3-6} 
swimming &  & \multicolumn{1}{l|}{0.818} & 0.613 & \multicolumn{1}{l|}{0.821} & 0.638 \\ \cline{1-1} \cline{3-6} 
reading &  & \multicolumn{1}{l|}{0.782} & 0.578 & \multicolumn{1}{l|}{0.769} & 0.469 \\ \cline{1-1} \cline{3-6} 
run &  & \multicolumn{1}{l|}{0.826} & 0.478 & \multicolumn{1}{l|}{0.822} & 0.395 \\ \cline{1-1} \cline{3-6} 
dancing &  & \multicolumn{1}{l|}{0.805} & 0.569 & \multicolumn{1}{l|}{0.908} & 0.828 \\ \cline{1-1} \cline{3-6} 
floating &  & \multicolumn{1}{l|}{0.789} & 0.596 & \multicolumn{1}{l|}{0.824} & 0.555 \\ \cline{1-1} \cline{3-6} 
feeding &  & \multicolumn{1}{l|}{0.788} & 0.627 & \multicolumn{1}{l|}{0.765} & 0.558 \\ \hline
blue & \multirow{8}{*}{adjective} & \multicolumn{1}{l|}{0.672} & 0.348 & \multicolumn{1}{l|}{0.708} & 0.452 \\ \cline{1-1} \cline{3-6} 
front &  & \multicolumn{1}{l|}{0.659} & 0.253 & \multicolumn{1}{l|}{0.706} & 0.213 \\ \cline{1-1} \cline{3-6} 
little &  & \multicolumn{1}{l|}{0.725} & 0.42 & \multicolumn{1}{l|}{0.748} & 0.448 \\ \cline{1-1} \cline{3-6} 
green &  & \multicolumn{1}{l|}{0.688} & 0.422 & \multicolumn{1}{l|}{0.715} & 0.421 \\ \cline{1-1} \cline{3-6} 
yellow &  & \multicolumn{1}{l|}{0.722} & 0.48 & \multicolumn{1}{l|}{0.742} & 0.521 \\ \cline{1-1} \cline{3-6} 
pink &  & \multicolumn{1}{l|}{0.718} & 0.519 & \multicolumn{1}{l|}{0.731} & 0.61 \\ \cline{1-1} \cline{3-6} 
navy &  & \multicolumn{1}{l|}{0.738} & 0.565 & \multicolumn{1}{l|}{0.768} & 0.685 \\ \cline{1-1} \cline{3-6} 
maroon &  & \multicolumn{1}{l|}{0.778} & 0.59 & \multicolumn{1}{l|}{0.844} & 0.684 \\ \hline
\end{tabular}

}
\end{center}

\label{tab:concept_description}

\end{table}


==> Table/cross_dataset.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{Cross-dataset targeted attack performance}. The results of training and test using different datasets are on the off-diagonal.}
\begin{center}
\scalebox{1.0}{

\begin{tabular}{|clll|}
\hline
\multicolumn{4}{|l|}{Model: CLIP} \\ \hline
\multicolumn{2}{|c|}{\multirow{2}{*}{mAP}} & \multicolumn{2}{c|}{test dataset} \\ \cline{3-4} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{l|}{Flickr} & MSCOCO \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}training\\  dataset\end{tabular}}} & \multicolumn{1}{l|}{Flickr} & \multicolumn{1}{l|}{0.805} & 0.558 \\ \cline{2-4} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{MSCOCO} & \multicolumn{1}{l|}{0.622} & 0.597 \\ \hline
\multicolumn{4}{|l|}{Model: {\clipF}} \\ \hline
\multicolumn{2}{|c|}{\multirow{2}{*}{mAP}} & \multicolumn{2}{c|}{test dataset} \\ \cline{3-4} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{l|}{Flickr} & MSCOCO \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}training\\  dataset\end{tabular}}} & \multicolumn{1}{l|}{Flickr} & \multicolumn{1}{l|}{0.547} & 0.216 \\ \cline{2-4} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{MSCOCO} & \multicolumn{1}{l|}{0.404} & 0.299 \\ \hline
\multicolumn{4}{|l|}{Model: {\clipC}} \\ \hline
\multicolumn{2}{|c|}{\multirow{2}{*}{mAP}} & \multicolumn{2}{c|}{test dataset} \\ \cline{3-4} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{l|}{Flickr} & MSCOCO \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}training\\  dataset\end{tabular}}} & \multicolumn{1}{l|}{Flickr} & \multicolumn{1}{l|}{0.580} & 0.347 \\ \cline{2-4} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{MSCOCO} & \multicolumn{1}{l|}{0.451} & 0.352 \\ \hline
\end{tabular}

}
\end{center}

\label{tab:cross_dataset}

\end{table}


==> Table/cross_model.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{Cross-model targeted attack performance}. The results of training and test using different models are on the off-diagonal.}
\begin{center}
\scalebox{1.0}{

\begin{tabular}{|cllll|}
\hline
\multicolumn{5}{|l|}{Dataset: Flickr} \\ \hline
\multicolumn{2}{|c|}{\multirow{2}{*}{mAP}} & \multicolumn{3}{c|}{test model} \\ \cline{3-5} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{l|}{CLIP} & \multicolumn{1}{l|}{{\clipF}} & {\clipC} \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}training\\  model\end{tabular}}} & \multicolumn{1}{l|}{CLIP} & \multicolumn{1}{l|}{0.805} & \multicolumn{1}{l|}{0.178} & 0.115 \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{{\clipF}} & \multicolumn{1}{l|}{0.109} & \multicolumn{1}{l|}{0.542} & 0.416 \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{{\clipC}} & \multicolumn{1}{l|}{0.109} & \multicolumn{1}{l|}{0.450} & 0.580 \\ \hline
\multicolumn{5}{|l|}{Dataset: COCO} \\ \hline
\multicolumn{2}{|c|}{\multirow{2}{*}{mAP}} & \multicolumn{3}{c|}{test model} \\ \cline{3-5} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{l|}{CLIP} & \multicolumn{1}{l|}{{\clipF}} & {\clipC} \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}training\\  model\end{tabular}}} & \multicolumn{1}{l|}{CLIP} & \multicolumn{1}{l|}{0.597} & \multicolumn{1}{l|}{0.056} & 0.062 \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{{\clipF}} & \multicolumn{1}{l|}{0.068} & \multicolumn{1}{l|}{0.299} & 0.217 \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{{\clipC}} & \multicolumn{1}{l|}{0.053} & \multicolumn{1}{l|}{0.211} & 0.352 \\ \hline
\end{tabular}

}
\end{center}

\label{tab:cross_model}

\end{table}


==> Table/dataset_statistics.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{Statistics on the number of images in Flickr30k and MSCOCO}. Each image is described with five related sentences.}
\begin{center}
\setlength{\tabcolsep}{3mm}{ 

\begin{tabular}{@{}lrrr@{}}
\toprule
\textbf{Dataset} & \multicolumn{1}{l}{\textbf{Training}} & \multicolumn{1}{l}{\textbf{Validation}} & \multicolumn{1}{l}{\textbf{Test}} \\ \midrule
Flickr30k & 29783 & 1000 & 1000 \\
MSCOCO & 122287 & 5000 & 5000 \\ \bottomrule
\end{tabular}

}


\end{center}

\label{tab:dataset_statistics}

\end{table}


==> Table/related_works.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{An summary of previous works on attacking deep-learning image retrieval}. By inserting targeted Toran-horse images into the database of a language-based image retrieval system, this paper differs from the prior works in two aspects, \ie query modality and attack point.  }
\begin{center}
\begin{threeparttable}
\setlength{\tabcolsep}{6mm}{ 
 
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Method} & \textbf{Query modality} & \textbf{Attack point} & \textbf{Attack range} & \textbf{Targeted} \\ \midrule
PIRE, ICMR19 \cite{liu2019s} & Image & Front-end & Single query & No \\
TMAA, ICCV19 \cite{tolias2019targeted} & Image & Front-end & Single query & Yes \\
CMLA, NIPS19 \cite{LiGDXL19_nips} & Tag & Front-end & Single query & No \\
UAA-GAN, arXiv19 \cite{zhao2019unsupervised} & Image & Front-end & Single query & No \\
% AP-GAN, arXiv20 \cite{zhao2020ap} & Image & Front-end& Single query & No \\
DAIR, SIGIR21 \cite{chen2021dair} & Image & Front-end & Single query & No \\
AACH, ICCV21 \cite{Li_2021_ICCV} & Tag & Front-end & Single query & No \\
AdvHash, MM21 \cite{hu2021advhash} & Image &Front-end & Query set & Yes \\

\emph{This paper} & \textit{Sentence} & \textit{Back-end} & Query set & Yes \\ \bottomrule
\end{tabular}

}

\end{threeparttable}


\end{center}

\label{tab:related_works}

\end{table*}


==> Table/result_all_R10.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{R10 of LBIR system without/with {\TTHImage} images \wrt specific queries in three different TTH attack modes, \ie white-box attack, surrogate-dataset attack and surrogate-model attack.} Surrogate-dataset is training and evaluation with different datasets. Surrogate-model is training and evaluation with different models.}
\begin{center}
\scalebox{1.0}{
% \setlength{\tabcolsep}{3mm}{ 

\begin{tabular}{@{}llllllrrrrr@{}}
\toprule
\multicolumn{2}{l}{\textbf{TTH attack setup}} & \textbf{} & \multicolumn{2}{l}{\textbf{LBIR configuration}} & \textbf{} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Truly relevant \\ images\end{tabular}}} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{2}{c}{\textbf{{\TTHImage} images}} \\ \cline{1-2} \cline{4-5} \cline{7-8} \cline{10-11} 
\textit{Network} & \textit{Training data} & \textit{} & \textit{Network} & \textit{Image set} & \textit{} & \textit{w/o TTH} & \textit{w/ TTH} & \textit{} & \textit{w/o TTH} & \textit{w/ TTH} \\ \midrule
% \multicolumn{11}{l}{\textit{\textbf{White-box attack}}} \\ 
{\textit{\textbf{White-box attack}}} \\ 
CLIP & Flickr30k-train &  & CLIP & Flickr30k-test &  & 94.9 & 52.1 &  & 0.0 & 97.2 \\
{\clipF} & Flickr30k-train &  & {\clipF} & Flickr30k-test &  & 98.6 & 95.3 &  & 0.8 & 77.1 \\
CLIP & COCO-train &  & CLIP & COCO-test &  & 80.5 & 51.2 &  & 0.0 & 82.3 \\
{\clipC} & COCO-train &  & {\clipC} & COCO-test &  & 90.1 & 83.9 &  & 1.8 & 44.9 \\
\textit{\textbf{Surrogate-dataset Attack}} \\
CLIP & COCO-train &  & CLIP & Flickr30k-test &  & 94.9 & 70.5 &  & 0.0 & 83.1 \\
CLIP & Flickr30k-train &  & CLIP & COCO-test &  & 80.5 & 53.5 &  & 0.0 & 77.8 \\
{\clipF} & COCO-train &  & {\clipF} & Flickr30k-test &  & 98.6 & 97.7 &  & 0.8 & 58.6 \\
{\clipF} & Flickr30k-train &  & {\clipF} & COCO-test &  & 85.0 & 82.8 &  & 0.1 & 34.4 \\
{\clipC} & COCO-train &  & {\clipC} & Flickr30k-test &  &  97.5 & 94.8 &  & 0.9 & 69.2 \\
{\clipC} & Flickr30k-train &  & {\clipC} & COCO-test &  & 90.1 & 84.0 &  & 1.8 & 44.5 \\
% {\color[HTML]{2B2B2B} \textbf{Surrogate-model attack}} &  &  &  &  &  &  &  &  &  &  \\
{\textit{\textbf{Surrogate-model attack}}} \\
CLIP & Flickr30k-train &  & {\clipF} & Flickr30k-test &  & 97.8 & 97.8 &  & 0.8 & 18.5 \\
CLIP & COCO-train &  & {\clipC} & COCO-test &  & 90.1 & 90.1 &  & 1.8 & 7.8 \\
{\clipF} & COCO-train &  & {\clipC} & COCO-test &  & 90.1 & 87.1 &  & 1.8 & 37.5 \\
{\clipC} & Flickr30k-train &  & {\clipF} & Flickr30k-test &  & 98.6 & 97.2 &  & 0.8 & 70.6 \\ \bottomrule
\end{tabular}

% }
}
\end{center}

\label{tab:result_all_R10}

\end{table*}


==> Table/result_coco_clip.tex <==

\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
%R10 of truly relevant images and {\TTHImage} images \wrt specific queries
\caption{\textbf{R10 of LBIR system without/with {\TTHImage} images \wrt specific queries}. LBIR  setup: CLIP + COCOtest. 
% Adversarial patches are learned with COCOtrain as the training data.
}
\begin{center}
\scalebox{0.9}{

\begin{tabular}{@{}lrrlrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Query set}}} & \multicolumn{2}{c}{\textbf{Truly relevant images}} &  & \multicolumn{2}{c}{\textbf{Benign or {\TTHImage} images}} \\ \cline{2-3} \cline{5-6} 
\multicolumn{1}{c}{} & \multicolumn{1}{l}{\textit{\textbf{w/o TTH}}} & \multicolumn{1}{l}{\textit{\textbf{w/ TTH}}} &  & \multicolumn{1}{l}{\textit{\textbf{w/o TTH}}} & \multicolumn{1}{l}{\textit{\textbf{w/ TTH}}} \\ \midrule
waiter & 100.0 & 0.0 &  & 0.0 & 100.0 \\
policeman & 80.0 & 20.0 &  & 0.0 & 100.0 \\
dancing & 100.0 & 50.0 &  & 0.0 & 100.0 \\
floating & 68.4 & 18.4 &  & 0.0 & 100.0 \\
maroon & 100.0 & 60.0 &  & 0.0 & 100.0 \\
motorcycle & 62.7 & 31.5 &  & 0.0 & 98.1 \\
smiling & 77.6 & 35.8 &  & 0.0 & 97.8 \\
cow & 76.4 & 52.8 &  & 0.0 & 95.3 \\
pink & 89.7 & 68.4 &  & 0.0 & 94.1 \\
climbing & 94.1 & 58.8 &  & 0.0 & 88.2 \\
little & 82.4 & 34.5 &  & 0.0 & 87.9 \\
jacket & 75.0 & 53.1 &  & 0.0 & 87.5 \\
dress & 88.7 & 52.8 &  & 0.0 & 84.9 \\
navy & 83.3 & 66.7 &  & 0.0 & 83.3 \\
swimming & 93.5 & 78.3 &  & 0.0 & 80.4 \\
reading & 93.6 & 70.2 &  & 0.0 & 78.7 \\
female & 64.4 & 46.7 &  & 0.0 & 77.8 \\
run & 45.5 & 39.4 &  & 0.0 & 72.7 \\
yellow & 78.6 & 63.6 &  & 0.0 & 70.9 \\
blue & 75.0 & 60.4 &  & 0.0 & 65.5 \\
floor & 85.8 & 67.6 &  & 0.0 & 64.2 \\
feeding & 76.4 & 69.1 &  & 0.0 & 56.4 \\
front & 68.8 & 64.8 &  & 0.0 & 47.0 \\
green & 72.1 & 66.5 &  & 0.0 & 45.4 \\
\textbf{MEAN} & \textbf{80.5} & \textbf{51.2} &  & \textbf{0.0} & \textbf{82.3} \\ \midrule
\end{tabular}

}
\end{center}

\label{tab:result_coco_clip}

\end{table}


==> Table/result_coco_clipC.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
%R10 of truly relevant images and {\TTHImage} images \wrt specific queries
\caption{\textbf{R10 of LBIR system without/with {\TTHImage} images \wrt specific queries}. LBIR  setup: {\clipC} + COCOtest. 
% Adversarial patches are learned with COCOtrain as the training data.
}
\begin{center}
\scalebox{0.9}{

\begin{tabular}{@{}lrrlrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Query set}}} & \multicolumn{2}{c}{\textbf{Truly relevant images}} &  & \multicolumn{2}{c}{\textbf{Benign or {\TTHImage} images}} \\ \cline{2-3} \cline{5-6} 
\multicolumn{1}{c}{} & \multicolumn{1}{l}{\textit{\textbf{w/o TTH}}} & \multicolumn{1}{l}{\textit{\textbf{w/ TTH}}} &  & \multicolumn{1}{l}{\textit{\textbf{w/o TTH}}} & \multicolumn{1}{l}{\textit{\textbf{w/ TTH}}} \\ \midrule
waiter & 100.0 & 100.0 &  & 0.0 & 100.0 \\
policeman & 80.0 & 40.0 &  & 0.0 & 100.0 \\
dancing & 100.0 & 50.0 &  & 0.0 & 100.0 \\
navy & 83.3 & 83.3 &  & 0.0 & 83.3 \\
maroon & 80.0 & 60.0 &  & 20.0 & 80.0 \\
pink & 94.1 & 86.0 &  & 0.0 & 68.4 \\
reading & 97.9 & 91.5 &  & 6.4 & 57.4 \\
dress & 98.1 & 94.3 &  & 1.9 & 56.6 \\
motorcycle & 86.8 & 77.8 &  & 0.0 & 54.0 \\
cow & 90.6 & 86.6 &  & 0.0 & 45.7 \\
smiling & 95.5 & 94.0 &  & 0.7 & 44.0 \\
feeding & 89.1 & 89.1 &  & 1.8 & 38.2 \\
little & 93.1 & 92.4 &  & 0.3 & 37.9 \\
swimming & 97.8 & 97.8 &  & 0.0 & 32.6 \\
yellow & 92.4 & 92.0 &  & 1.2 & 30.6 \\
floating & 76.3 & 73.7 &  & 2.6 & 26.3 \\
floor & 92.0 & 90.9 &  & 1.1 & 25.6 \\
jacket & 89.1 & 89.1 &  & 0.0 & 25.0 \\
climbing & 94.1 & 94.1 &  & 0.0 & 23.5 \\
blue & 91.5 & 89.9 &  & 0.2 & 21.3 \\
green & 89.3 & 88.9 &  & 0.4 & 14.6 \\
front & 87.8 & 87.8 &  & 1.0 & 4.5 \\
female & 84.4 & 84.4 &  & 4.4 & 4.4 \\
run & 78.8 & 78.8 &  & 0.0 & 3.0 \\
\textbf{MEAN} & \textbf{90.1} & \textbf{83.9} &  & \textbf{1.8} & \textbf{44.9} \\ \midrule
\end{tabular}

}
\end{center}

\label{tab:result_coco_clipC}

\end{table}


==> Table/result_flick_clip.tex <==

\begin{table}[t!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
%R10 of truly relevant images and {\TTHImage} images \wrt specific queries
\caption{\textbf{R10 of LBIR system without/with {\TTHImage} images \wrt specific queries}.  LBIR  setup: CLIP + Flickr30ktest. 
% Adversarial patches are learned with Flickr30ktrain as training data. 
The clear drop of R10 for truley relevant images and the clear increase of R10 for {\TTHImage} images show the success of the proposed method for making TTH attacks.}
\begin{center}
\scalebox{0.9}{

\begin{tabular}{@{}lrrlrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Query set}}} & \multicolumn{2}{c}{\textbf{Truly relevant images}} &  & \multicolumn{2}{c}{\textbf{Benign or {\TTHImage} images}} \\ \cline{2-3} \cline{5-6} 
\multicolumn{1}{c}{} & \multicolumn{1}{l}{\textit{\textbf{w/o TTH}}} & \multicolumn{1}{l}{\textit{\textbf{w/ TTH}}} &  & \multicolumn{1}{l}{\textit{\textbf{w/o TTH}}} & \multicolumn{1}{l}{\textit{\textbf{w/ TTH}}} \\ \midrule
waiter & 100.0 & 20.0 &  & 0.0 & 100.0 \\
motorcycle & 90.5 & 28.6 &  & 0.0 & 100.0 \\
run & 92.3 & 30.8 &  & 0.0 & 100.0 \\
dress & 92.4 & 42.4 &  & 0.0 & 100.0 \\
floating & 90.0 & 40.0 &  & 0.0 & 100.0 \\
smiling & 94.6 & 48.2 &  & 0.0 & 100.0 \\
policeman & 100.0 & 58.3 &  & 0.0 & 100.0 \\
feeding & 100.0 & 60.0 &  & 0.0 & 100.0 \\
maroon & 100.0 & 60.0 &  & 0.0 & 100.0 \\
navy & 100.0 & 66.7 &  & 0.0 & 100.0 \\
cow & 100.0 & 73.3 &  & 0.0 & 100.0 \\
little & 91.9 & 29.0 &  & 0.0 & 98.9 \\
swimming & 97.8 & 43.5 &  & 0.0 & 97.8 \\
climbing & 95.5 & 11.4 &  & 0.0 & 97.7 \\
blue & 95.4 & 61.4 &  & 0.0 & 97.3 \\
dancing & 80.0 & 33.3 &  & 0.0 & 96.7 \\
yellow & 93.2 & 68.9 &  & 0.0 & 96.3 \\
floor & 97.7 & 70.5 &  & 0.0 & 95.5 \\
reading & 94.7 & 52.6 &  & 0.0 & 94.7 \\
jacket & 91.4 & 69.9 &  & 0.0 & 94.6 \\
pink & 94.3 & 52.9 &  & 0.0 & 94.3 \\
green & 94.9 & 76.0 &  & 0.0 & 92.0 \\
female & 100.0 & 73.9 &  & 0.0 & 89.1 \\
front & 92.0 & 78.0 &  & 0.0 & 88.6 \\
\textbf{MEAN} & \textbf{94.9} & \textbf{52.1} &  & \textbf{0.0} & \textbf{97.2} \\ \midrule
\end{tabular}

}
\end{center}

\label{tab:result_flick_clip}

\end{table}


==> Table/result_flickr_clipF.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
\normalsize
\renewcommand\arraystretch{1.0}
\centering

\caption{\textbf{R10 of LBIR system without/with {\TTHImage} images \wrt specific queries}. LBIR  setup: {\clipF} + Flickr30ktest. 
% Adversarial patches are learned with Flickr30ktrain as training data. 
}
\begin{center}
\scalebox{0.9}{

\begin{tabular}{@{}lrrlrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Query set}}} & \multicolumn{2}{c}{\textbf{Truly relevant images}} &  & \multicolumn{2}{c}{\textbf{Benign or {\TTHImage} images}} \\ \cline{2-3} \cline{5-6} 
\multicolumn{1}{c}{} & \multicolumn{1}{l}{\textit{\textbf{w/o TTH}}} & \multicolumn{1}{l}{\textit{\textbf{w/ TTH}}} &  & \multicolumn{1}{l}{\textit{\textbf{w/o TTH}}} & \multicolumn{1}{l}{\textit{\textbf{w/ TTH}}} \\ \midrule
cow & 100.0 & 86.7 &  & 0.0 & 100.0 \\
motorcycle & 100.0 & 95.2 &  & 0.0 & 100.0 \\
policeman & 100.0 & 100.0 &  & 0.0 & 100.0 \\
waiter & 100.0 & 100.0 &  & 0.0 & 100.0 \\
feeding & 100.0 & 100.0 &  & 0.0 & 100.0 \\
reading & 94.7 & 86.8 &  & 0.0 & 97.4 \\
swimming & 100.0 & 100.0 &  & 0.0 & 91.3 \\
floor & 100.0 & 100.0 &  & 2.3 & 86.4 \\
dress & 100.0 & 95.5 &  & 1.5 & 86.4 \\
pink & 97.7 & 96.6 &  & 0.0 & 86.2 \\
climbing & 95.5 & 84.1 &  & 0.0 & 84.1 \\
smiling & 100.0 & 98.2 &  & 3.6 & 83.9 \\
dancing & 90.0 & 83.3 &  & 0.0 & 83.3 \\
yellow & 97.5 & 93.8 &  & 3.1 & 77.6 \\
green & 98.9 & 97.1 &  & 0.6 & 73.1 \\
floating & 100.0 & 90.0 &  & 0.0 & 70.0 \\
run & 100.0 & 92.3 &  & 0.0 & 69.2 \\
navy & 100.0 & 100.0 &  & 0.0 & 66.7 \\
little & 98.9 & 98.4 &  & 1.1 & 65.6 \\
female & 100.0 & 100.0 &  & 2.2 & 60.9 \\
jacket & 96.8 & 95.7 &  & 0.0 & 57.0 \\
blue & 98.2 & 97.9 &  & 1.2 & 41.6 \\
maroon & 100.0 & 100.0 &  & 0.0 & 40.0 \\
front & 97.3 & 96.6 &  & 4.2 & 29.9 \\
\textbf{MEAN} & \textbf{98.6} & \textbf{95.3} &  & \textbf{0.8} & \textbf{77.1} \\ \midrule
\end{tabular}

}
\end{center}

\label{tab:result_flick_clipF}

\end{table}


==> Table/retrieval_models.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{The state-of-the-arts of text to image retrieval in Flickr30k}. }
\begin{center}
\scalebox{0.9}{

\begin{tabular}{|l|lll|lll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{Flickr30k (1K test)} & \multicolumn{3}{c|}{MSCOCO2014 (5K test)} \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{l|}{R1} & \multicolumn{1}{l|}{R5} & R10 & \multicolumn{1}{l|}{R1} & \multicolumn{1}{l|}{R5} & R10 \\ \hline
VSE++ \cite{2018vse_plus} & \multicolumn{1}{l|}{39.6} & \multicolumn{1}{l|}{70.1} & 79.5 & \multicolumn{1}{l|}{30.3} & \multicolumn{1}{l|}{59.4} & 72.4 \\ \hline
SGRAF \cite{2021_sgraf} & \multicolumn{1}{l|}{58.5} & \multicolumn{1}{l|}{83} & 88.8 & \multicolumn{1}{l|}{41.9} & \multicolumn{1}{l|}{70.7} & 81.3 \\ \hline
ViLT-B/32 \cite{2021_vilt_KimSK21} & \multicolumn{1}{l|}{64.4} & \multicolumn{1}{l|}{88.7} & 93.8 & \multicolumn{1}{l|}{42.7} & \multicolumn{1}{l|}{72.9} & 83.1 \\ \hline
CLIP \cite{2021clip_icml} & \multicolumn{1}{l|}{68.7} & \multicolumn{1}{l|}{90.6} & 95.2 & \multicolumn{1}{l|}{37.8} & \multicolumn{1}{l|}{62.4} & 72.2 \\ \hline
CLIP-FT \cite{hu2021lightweight} & \multicolumn{1}{l|}{75.2} & \multicolumn{1}{l|}{93.5} & 96.2 & \multicolumn{1}{l|}{45.6} & \multicolumn{1}{l|}{72.9} & 82.2 \\ \hline
ALIGN \cite{2021_icml_align} & \multicolumn{1}{l|}{84.9} & \multicolumn{1}{l|}{97.4} & 98.6 & \multicolumn{1}{l|}{59.9} & \multicolumn{1}{l|}{82.8} & 89.8 \\ \hline
\end{tabular}

}
\end{center}

\label{tab:retrieval_models}

\end{table}


==> backup.tex <==
When a retrieval system expands data, its database is at risk of being attacked. In this paper, we introduce the method of targeted Trojan-horse ({\ModelName}) attack for language-based image retrieval (LBIR), the first {\TargetedObject}-wise targeted attack against the database of retrieval system. Specifically, given a specific \djf{target} {\TargetedObject}, \ModelName generates a QR-code patch that can be applied to a set of different images to gain the targeted Trojan-horse images, which closes to \djf{the} target {\TargetedObject} in the common space of cross-modal matching of retrieval model. 
When a database is poisoned by \ModelName attack, \ModelName images will be highly ranked 
% will \djf{be} rank\djf{ed} high
in a normal search, even though the images are completely irrelevant to the query. 
\djf{Extensive experimental results on two language-based image retrieval benchmarks (\ie Flickr30k and MSCOCO), have shown the effectiveness of our proposed attack method under two attack settings, \ie white-box and cross-dataset attacks.}
% We evaluate the attacks on standard language-based image retrieval benchmarks (i.e. Flickr30k and MSCOCO) and compare the results retrieved with and without the Trojan-horse images. 



In this paper, we propose targeted \textbf{T}rojan-\textbf{H}orse \textbf{A}ttack (\ModelName) on Language-based Image retrieval,  where one single patch with targeted {\TargetedObject}s information can be effectively applied to a set of image samples to cause the mismatch when queries contain the targeted {\TargetedObject}s. 
% Different from the attack method\djf{s} of disturbing the query, 
As summarized in \cref{tab:related_works}, {\ModelName} is the first back-end attack, which breaks the return list by poisoning the retrieval database with adversarial images. 
Moreover, the attack in {\ModelName} is targeted, \ie {\ModelName} aims to make the adversarial images ranking as high as possible when retrieving queries including targeted {\TargetedObject}. We formulate this as an images-to-{\TargetedObject} problem and design \djf{a} loss function to increase the cosine similarity between embeddings of adversarial images and the contextualized embedding of the given {\TargetedObject}. We use the average embedding of different sentences containing targeted {\TargetedObject} to represent the contextualized embedding. Then we use the gradient descent method to optimize the patch. 


For image-to-image retrieval, different approaches such as PIRE \cite{liu2019s}, UAA-GAN \cite{zhao2019unsupervised}, and AP-GAN \cite{zhao2020ap} have been proposed to realize non-targeted image-specific attack. TMAA \cite{tolias2019targeted} is the first targeted attack against image-to-image retrieval and AdvHash \cite{hu2021advhash} extends the targeted attack to class-wise scenario, where the attack method is effective to all queries which belong to a specific class. DAIR \cite{chen2021dair} explores a query-efficient decision-based black-box attack against image retrieval. For cross-modal retrieval by hamming distance, Li et al. \cite{LiGDXL19_nips} first explore tag-to-image adversarial samples in white-box setting and then AACH \cite{Li_2021_ICCV} is proposed to investigate the black-box setting. 



As summarized in Tab. \ref{tab:related_works}, attack on sentence query modality remains unexplored. Whether it is an attack on image retrieval or tag-to-image retrieval, the usual approach is to push the feature embedding of the target query away from its original region in the feature space. In this way, the images related to the query will not appear in the top list returned by the retrieval. However, these attacks present the same shortcomings: they require test-time queries to be modified to trigger the attack. Our attack aims to let the searcher see the image specified by the attacker without query modification. 


\begin{table}[tbh!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
% \arrayrulecolor{red}
\normalsize
\renewcommand\arraystretch{1.0}
\centering
\caption{\textbf{An summary of previous works on attacking deep-learning image retrieval}. By inserting targeted Toran-horse images into the database of a language-based image retrieval system, this paper differs from the prior works in two aspects, \ie query modality and attack point.  }
\begin{center}
\scalebox{0.7}{
\setlength{\tabcolsep}{1mm}{ 
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Method} & \textbf{Query modality} & \textbf{Attack point} & \textbf{Attack range} & \textbf{Targeted} \\ \midrule
PIRE, ICMR19 \cite{liu2019s} & Image & Front-end & Single query & No \\
TMAA, ICCV19 \cite{tolias2019targeted} & Image & Front-end & Single query & Yes \\
CMLA, NIPS19 \cite{LiGDXL19_nips} & Tag & Front-end & Single query & No \\
UAA-GAN, arXiv19 \cite{zhao2019unsupervised} & Image & Front-end & Single query & No \\
% AP-GAN, arXiv20 \cite{zhao2020ap} & Image & Front-end& Single query & No \\
DAIR, SIGIR21 \cite{chen2021dair} & Image & Front-end & Single query & No \\
AACH, ICCV21 \cite{Li_2021_ICCV} & Tag & Front-end & Single query & No \\
AdvHash, MM21 \cite{hu2021advhash} & Image &Front-end & Query set & Yes \\

\emph{This paper} & \textit{Sentence} & \textit{Back-end} & Query set & Yes \\ \bottomrule
\end{tabular}
}
}

\end{center}
\label{tab:related_works}
\end{table}



\begin{figure}
  \begin{subfigure}{0.49\linewidth} % 如果一行放2个图，用0.5，如果3个图，用0.33
    \centering 
    \includegraphics[scale=0.25]{Image/policeman_Tsne_result.jpg} 
    \caption{policeman}
    \label{fig:tsne_policeman}
  \end{subfigure}
  \begin{subfigure}{0.49\linewidth}
    \centering 
    \includegraphics[scale=0.25]{Image/swimming_Tsne_result.jpg} 
    \caption{swimming}
    \label{fig:tsne_swimming}
  \end{subfigure}
  
  \begin{subfigure}{0.49\linewidth}
    \centering 
    \includegraphics[scale=0.25]{Image/front_Tsne_result.jpg} 
    \caption{front}
    \label{fig:tsne_front}
  \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
    \centering 
    \includegraphics[scale=0.25]{Image/run_Tsne_result.jpg} 
    \caption{run}
    \label{fig:tsne_runs}
  \end{subfigure}
  
 \caption{\textbf{Visualization of {\clipF} model embbedings of four {\TargetedObject}s in Flickr30Ktest. } Grey dots, purple dots, and yellow dots mean all images in test dataset, texts including targeted {\TargetedObject}  in test dataset and trojan-horse images. }
  \label{Figure:tsne_four_concepts}
\end{figure}


The detailed R10 results of truly relevant images and {\TTHImage} images \wrt specific queries is shown in \cref{tab:result_flick_clipF}. The order of {\TargetedObject} is in descending order according to the R10 increase of {\TTHImage} images before and after attacking. We observe that there is a large difference in the attack performance of different {\TargetedObject}s. We assume that some {\TargetedObject}s, such as \textit{front}, are composed of sentences with rich meanings and sparse meaning distribution in the model subspace, so it is more difficult to construct a unified patch to attack. To prove the assumption, we select two {\TargetedObject}s (policeman and swimming) with good attack effects and two {\TargetedObject}s (front and run) with poor attack effects. As depicted in Fig. \ref{Figure:tsne_four_concepts}, we visualize {\clipF} subspace embeddings of all images in flickr30k test dataset, texts including targeted {\TargetedObject} in flickr30k test dataset and {\TTHImage} images. Because the embeddings of "front" and "run" are scattered in the subspace, it is difficult to put the embeddings of {\TTHImage} images and all texts including "front" or "run" in the subspace close to each other.



\begin{figure*}
    \subfloat[The influence of $\mathbf{\lambda}$. \label{fig:qr_adjust_lam}]{\includegraphics[width=0.75\columnwidth]{Image/qr_adjust_lam.pdf}} 
    \subfloat[The visualization of patch size. \label{fig:visualization_adjust_ratio}]{\includegraphics[width=0.75\columnwidth]{Image/visualization_adjust_ratio.pdf}} 
    \subfloat[The influence of patch size. \label{fig:adjust_ratio}]{\includegraphics[width=0.45\columnwidth]{Image/adjust_ratio.pdf}} 
    
    \caption{{Ablation study of different $\mathbf{\lambda}$ and patch size.} LBIR  setup: {\clipF} + Flickr30ktest.}
    \label{Figure:adjust_lambda_and_radio}
\end{figure*}



\begin{table}[t!]
\setlength{\abovecaptionskip}{0.cm}
\setlength{\belowcaptionskip}{-0.cm}
\normalsize
\renewcommand\arraystretch{1.0}
\centering

\caption{\textbf{R10 of LBIR system without/with {\TTHImage} images \wrt specific queries}. LBIR  setup: {\clipF} + Flickr30ktest. The R10 results of other LBIR setups can be found in our replication package.
}
\begin{center}
\scalebox{0.9}{

\begin{tabular}{@{}lrrlrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Query set}}} & \multicolumn{2}{c}{\textbf{Truly relevant images}} &  & \multicolumn{2}{c}{\textbf{Benign or {\TTHImage} images}} \\ \cline{2-3} \cline{5-6} 
\multicolumn{1}{c}{} & \multicolumn{1}{l}{\textit{\textbf{w/o \ModelName}}} & \multicolumn{1}{l}{\textit{\textbf{w/ \ModelName}}} &  & \multicolumn{1}{l}{\textit{\textbf{w/o \ModelName}}} & \multicolumn{1}{l}{\textit{\textbf{w/ \ModelName}}} \\ \midrule
cow & 100.0 & 86.7 &  & 0.0 & 100.0 \\
motorcycle & 100.0 & 95.2 &  & 0.0 & 100.0 \\
policeman & 100.0 & 100.0 &  & 0.0 & 100.0 \\
waiter & 100.0 & 100.0 &  & 0.0 & 100.0 \\
feeding & 100.0 & 100.0 &  & 0.0 & 100.0 \\
reading & 94.7 & 86.8 &  & 0.0 & 97.4 \\
swimming & 100.0 & 100.0 &  & 0.0 & 91.3 \\
floor & 100.0 & 100.0 &  & 2.3 & 86.4 \\
dress & 100.0 & 95.5 &  & 1.5 & 86.4 \\
pink & 97.7 & 96.6 &  & 0.0 & 86.2 \\
climbing & 95.5 & 84.1 &  & 0.0 & 84.1 \\
smiling & 100.0 & 98.2 &  & 3.6 & 83.9 \\
dancing & 90.0 & 83.3 &  & 0.0 & 83.3 \\
yellow & 97.5 & 93.8 &  & 3.1 & 77.6 \\
green & 98.9 & 97.1 &  & 0.6 & 73.1 \\
floating & 100.0 & 90.0 &  & 0.0 & 70.0 \\
run & 100.0 & 92.3 &  & 0.0 & 69.2 \\
navy & 100.0 & 100.0 &  & 0.0 & 66.7 \\
little & 98.9 & 98.4 &  & 1.1 & 65.6 \\
female & 100.0 & 100.0 &  & 2.2 & 60.9 \\
jacket & 96.8 & 95.7 &  & 0.0 & 57.0 \\
blue & 98.2 & 97.9 &  & 1.2 & 41.6 \\
maroon & 100.0 & 100.0 &  & 0.0 & 40.0 \\
front & 97.3 & 96.6 &  & 4.2 & 29.9 \\
\textbf{MEAN} & \textbf{98.6} & \textbf{95.3} &  & \textbf{0.8} & \textbf{77.1} \\ \midrule
\end{tabular}

}
\end{center}

\label{tab:result_flick_clipF}

\end{table}


\begin{figure}
    \subfloat[Attack performance. \label{fig:adjust_sigma_clip_F}]{\includegraphics[width=0.5\columnwidth]{Image/adjust_sigma_clip_F.pdf}} 
    \subfloat[Retrieval performance. \label{fig:adjust_sigma_clip_F_origin}]{\includegraphics[width=0.5\columnwidth]{Image/origin_adjust_sigma/clip_Flickr.pdf}} 
    
    \caption{{Attack performance (mean trojan-horse R10) and retrieval performance (mean Truly relevant R10) with different Gaussian's $\sigma$.} LBIR  setup: {\clipF} + Flickr30ktest.}
    \label{Figure:adjust_sigma}
\end{figure}

\subsection{Sensitivity to Gaussian blur} \label{ssec:gaussian}
Gaussian blur can also be used as an adversarial attack defense method~\cite{gu2019detecting, icic_WangWL21}. In this subsection, we analyze the sensitivity of our proposed {\ModelName} under different Gaussian blur settings.

% Gaussian blur (also known as Gaussian smoothing) is a common image pre-processing way, which could be used to reduce image noise and enhance image structures at different scale~\cite{gedraite2011investigation, singhal2017study, waltz1998efficient}. Gaussian blur can also be used as an adversarial attack defense method~\cite{gu2019detecting, icic_WangWL21}. The formula of a Gaussian function in two dimensions is
% \begin{equation}
% G(x, y)=\frac{1}{2 \pi \sigma^{2}} e^{-\frac{x^{2}+y^{2}}{2 \sigma^{2}}}, 
% \end{equation}
% where $x$ is the distance from the origin in the horizontal axis, $y$ is the distance from the origin in the vertical axis, and $\sigma$ is the standard deviation of the Gaussian distribution. As pixels at a distance of more than $3\sigma$ have a small enough influence to be considered effectively zero. We only calculate a matrix with dimensions $\lceil 6 \sigma\rceil \times\lceil 6 \sigma\rceil$ (where $\lceil\cdot\rceil$ is the ceiling function).

We set $\sigma$ from 0 to 10. The attack performance is shown on \cref{fig:adjust_sigma_clip_F}. We observe that the R10 of {\TTHImage} images decreases as $\sigma$ increases. What's more, a large $\sigma$ ($\sigma > 2$) has obvious effect on attack performance, which proves that a strong Gaussian blur can defend against {\ModelName} attack. However, large $\sigma$ ($\sigma > 2$) greatly decreases the retrieval accuracy, see \cref{fig:adjust_sigma_clip_F_origin}. Strong Gaussian blur also has obvious visual impact on original images, and the visualization can be found in our replication package. Therefore, it is unrealistic to use a strong Gaussian blur for {\ModelName} defense. 


\subsection{Ablation Study} \label{ssec:abaltion}
To explore the influence of $\lambda$ and the patch size, we make two ablation studies on CLIP+Flickr30ktest LBIR setup. All other experiment settings remain unchanged as  \cref{ssec:exp-setup}.

\textbf{The influence of $\mathbf{\lambda}$}. 
Take \textit{motorcycle} for example, the $\lambda$ is set to 0, 0.1, 0.3, 1 and 10, respectively. \cref{fig:qr_adjust_lam} shows R10 of {\TTHImage} images and whether QRcode is scannable with the increase of $\lambda$, it can be seen that  adversarial patch (QR-code) gradually becomes clear with the increase of $\lambda$ from 0 to 1, but R10 unaffected. On the other hand, when set $\lambda \geq 0.3 $, QR code is scannable.


\textbf{The influence of the patch size}. \cref{fig:adjust_ratio} shows the changing of R10 of {\TTHImage} images as the adversarial patch size increases. It can be seen that as the patch percentage increases, R10 increases accordingly. When the ratio is greater than 0.1, the performance improvement is relatively flat.
What's more, a large adversarial patch size would obscure the main part of the advertisement image, see \cref{fig:visualization_adjust_ratio}. To balance the effect of advertisement and attack performance, we set the patch ratio to 0.1.


